When AVSR Meets Video Conferencing: Dataset, Degradation, and the Hidden Mechanism Behind Performance Collapse

Audio-Visual Speech Recognition (AVSR) has achieved remarkable progress in offline conditions, yet its robustness in real-world video conferencing (VC) remains largely unexplored. This paper presents the first systematic evaluation of state-of-the-art AVSR models across mainstream VC platforms, revealing severe performance degradation caused by transmission distortions and spontaneous human hyper-expression. To address this gap, we construct \textbf{MLD-VC}, the first multimodal dataset tailored for VC, comprising 31 speakers, 22.79 hours of audio-visual data, and explicit use of the Lombard effect to enhance human hyper-expression. Through comprehensive analysis, we find that speech enhancement algorithms are the primary source of distribution shift, which alters the first and second formants of audio. Interestingly, we find that the distribution shift induced by the Lombard effect closely resembles that introduced by speech enhancement, which explains why models trained on Lombard data exhibit greater robustness in VC. Fine-tuning AVSR models on MLD-VC mitigates this issue, achieving an average 17.5% reduction in CER across several VC platforms. Our findings and dataset provide a foundation for developing more robust and generalizable AVSR systems in real-world video conferencing. MLD-VC is available at https://huggingface.co/datasets/nccm2p2/MLD-VC.

==> sec/0_abstract.tex <==
\begin{abstract}
Audio-Visual Speech Recognition (AVSR) has achieved remarkable progress in offline conditions, yet its robustness in real-world video conferencing (VC) remains largely unexplored. This paper presents the first systematic evaluation of state-of-the-art AVSR models across mainstream VC platforms, revealing severe performance degradation caused by transmission distortions and spontaneous human hyper-expression. To address this gap, we construct \textbf{MLD-VC}, the first multimodal dataset tailored for VC, comprising 31 speakers, 22.79 hours of audio-visual data, and explicit use of the Lombard effect to enhance human hyper-expression. Through comprehensive analysis, we find that speech enhancement algorithms are the primary source of distribution shift, which alters the first and second formants of audio. Interestingly, we find that the distribution shift induced by the Lombard effect closely resembles that introduced by speech enhancement, which explains why models trained on Lombard data exhibit greater robustness in VC. Fine-tuning AVSR models on MLD-VC mitigates this issue, achieving an average 17.5\% reduction in CER across several VC platforms. Our findings and dataset provide a foundation for developing more robust and generalizable AVSR systems in real-world video conferencing. MLD-VC is available at \href{https://huggingface.co/datasets/nccm2p2/MLD-VC}{https://huggingface.co/datasets/nccm2p2/MLD-VC}.

\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}
Audio-Visual Speech Recognition (AVSR) \cite{auto-avsr-1,auto-avsr-2,avsr_llm_1,robust_avsr_1} integrates audio and visual modalities to effectively overcome the performance limitations of single-modality Automatic Speech Recognition (ASR) \cite{asr_1,asr_2,asr_3,asr_4} under noisy or degraded conditions. It has become an important research direction for robust speech understanding. With the advancement of deep learning, state-of-the-art (SOTA) AVSR models have achieved remarkable performance on existing datasets. Since the outbreak of the COVID-19 pandemic, video conferencing (VC) platforms such as Zoom, Lark, Tencent Meeting, and DingTalk have become the primary means of remote communication. Consequently, AVSR has shown increasing demand in meeting transcription and accessibility support applications. 

\begin{figure}[t]
  \centering
   \includegraphics[width=1\linewidth]{sec/pictures/application.pdf}
   \caption{Compared to the face-to-face scenario, we identify two key factors affecting AVSR in video conferencing: transmission distortions in online and hyper-expression in a hindered communication environment.}
   \label{application}
\end{figure}

Most studies on robust AVSR \cite{robust_avsr_1,robust_avsr_2,robust_avsr_3,robust_avsr_4,robust_avsr_5} focus on noisy conditions or modality loss. However, our systematic evaluation reveals a critical issue: AVSR models experience severe performance degradation in VC, where the Word Error Rate (WER) and Character Error Rate (CER) increase from 0.93\%/0.56\% to 33.09\%/33.01\%. This collapse stems from the lack of datasets that reflect real-world VC conditions, as existing robustness studies are primarily conducted in offline or simulated environments, which fail to capture the complexity of real-world usage. As shown in Fig.~\ref{application}, communication in VC occurs through a camera and a display. This setting prompts participants to implicitly assume that the ongoing interaction is more constrained than face-to-face communication, leading them to adjust their communicative behaviors spontaneously. In addition, both audio and visual signals undergo compression, noise suppression, and speech enhancement during transmission, which introduces distortions to the data.

In this paper, we present the first systematic evaluation of mainstream AVSR models in VC, construct the first multimodal dataset covering multiple platforms, and reveal the issue of acoustic feature drift through a detailed analysis of the proposed dataset. By evaluating AVSR models across various VC platforms and datasets, we find consistent performance degradation across platforms, modalities, and languages, highlighting the universality of this problem. Based on the evaluation results and analysis, we identify two key factors responsible for the degradation of AVSR performance in VC: transmission distortions and spontaneous human hyper-expression \cite{hyper_1,hyper_theory}. To bridge the research gap in VC, we construct the first multimodal dataset for video conferencing (MLD-VC). MLD-VC comprises 31 speakers and 22 hours of recordings covering four mainstream VC platforms, with audio, video, and lip landmark data. Moreover, MLD-VC explicitly incorporates the Lombard effect to enhance and capture the manifestation of hyper-expression in VC. Experimental results show that fine-tuning AVSR models on MLD-VC reduces the average CER by 17.5\% in VC.

We summarize the main contributions of this paper as follows.
\begin{enumerate}
    \item [1)] \textbf{Conducting the First Systematic Evaluation in VC.} We conduct the first systematic evaluation of AVSR models in VC, revealing the widespread nature of performance degradation. We further identify two key contributing factors to this degradation: transmission distortions and spontaneous human hyper-expression.

    \item [2)] \textbf{Constructing the First Multimodal VC Dataset for AVSR.} We construct the first multimodal dataset captured directly through multiple real VC platforms (MLD-VC), which not only considers the real-world VC scenario but also incorporates the Lombard effect to enhance the hyper-expression. MLD-VC comprises 4 mainstream VC platforms, 31 speakers, and 22.79 hours of audio-visual recordings. 

    \item [3)] \textbf{Revealing the Hidden Mechanism Behind Performance Collapse.} We reveal that the fundamental cause of AVSR performance degradation in VC is feature distribution shift. We further demonstrate that speech enhancement algorithms are the primary factor driving the shift in audio distributions. In addition, we find that landmark-level features in the visual modality remain stable in VC, providing new insights for current AVSR visual encoders that rely on the unstable image-level representations.

    \item [4)] \textbf{Improving AVSR Performance in VC.} After fine-tuning the AVSR model on MLD-VC, we achieve an average reduction of 17.5\% in CER across several VC platforms. The ablation results show that the two key contributing factors are indispensable for improving model performance.
\end{enumerate}


==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
The columns should be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered, and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

The captions of the figures and tables should be in 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centered.  Table captions should be above tables, while figure captions should be below figures.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period, and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use the footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example, at the beginning of the sentence, you can use
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, include the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When citing multiple papers at once, make sure that you cite them in numerical order such as this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \caption{Results.   Ours is better.}
  \label{tab:example}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead, use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise and, therefore, must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it is almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence, avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/2_related_work.tex <==
\section{Related Work}
\subsection{Audio-Visual Speech Recognition}
AVSR \cite{avsr_1,avsr_2,avsr_3,avsr_4,avsr_5,avsr_6,avsr_7,auto-avsr-1,auto-avsr-2,avsr_llm_1,avsr_llm_2,avsr_llm_3,avsr_llm_4} integrates visual and acoustic features to enhance recognition accuracy under challenging and interference-prone conditions. Most existing studies on AVSR primarily focus on model robustness under noisy conditions or modality degradation \cite{robust_avsr_1,robust_avsr_2,robust_avsr_3,robust_avsr_4,robust_avsr_5}. 

Since the outbreak of the COVID-19 pandemic, AVSR systems have been widely adopted in VC scenarios. In such scenarios, besides background noise and modality loss, audio-visual streams are further affected by compression distortion and the spontaneous human hyper-expression \cite{hyper_1}. These factors introduce challenges that extend beyond traditional noise-robust settings, yet remain largely overlooked by current research. Most existing works still rely on pre-collected and tightly synchronized datasets, without accounting for the compression artifacts and hyper-expression behaviors commonly observed in VC \cite{hyper_1}. Consequently, the generalization of existing robust AVSR methods to real-world VC scenarios remains severely limited. However, there is currently a lack of datasets for AVSR robustness in VC scenarios.

\subsection{Human Hyper-expression}
Hyper-expression refers to a speaker’s compensatory behavior when communication is hindered \cite{hyper_1,hyper_theory, lombard_2,lombard_3,lombard_4}. In such cases, the speaker tends to increase vocal intensity, exaggerate facial expressions, and use more gestures to enhance intelligibility. Lindblom et al. \cite{hyper_theory} proposed the hyper/hypo theory, which explains the underlying mechanism of hyper-expression. According to this theory, speakers continuously evaluate the communicative environment to adjust their articulations dynamically in response to contextual demands. A typical form of hyper-expression is the Lombard effect, which occurs when speakers attempt to communicate in noisy environments \cite{lombard_2,lombard_3,lombard_4,lombard_avsr_1,lombard_avsr_2}. 
% In addition, the work of Trujillo et al. \cite{lombard_vision} demonstrated that hyper-expression can also be triggered by visual disturbances, suggesting that both visual and acoustic interferences can jointly elicit such behavior.

Russell et al. \cite{hyper_1} further showed that hyper-expression is prevalent in VC scenarios. By analyzing real-world Zoom meeting recordings, they found that participants exhibited hyper-expression, which is similar to the Lombard effect. The specific characteristics are more frequent pauses, longer vowel durations, and higher fundamental frequency values. These findings suggest that the performance degradation of AVSR models in VC scenarios is not solely attributed to the online communication setting, but also stems from the spontaneous hyper-expression of speakers.

==> sec/3__Evaluating_the_AVSR_Performance_in_Video_Meeting_Platforms.tex <==
\section{AVSR Performance in Video Conferencing}
\begin{table*}[htbp]
  \centering
  \caption{Performance of AVSR models on video conferencing platforms. “Offline” refers to the original dataset. “*” indicates that the corresponding metric is not applicable or not reported. “$\Delta$” refers to the absolute difference between VC platforms and Offline. Bold indicates the least change for each platform.}
  \label{avsr_results}
  \scalebox{0.7}{
  \setlength{\tabcolsep}{5pt}
  \begin{tabular}{ccccccccc}
    \toprule
    \textbf{Model} & \textbf{Dataset} & \textbf{Modal} & \textbf{Language} & \textbf{Platform} & \textbf{WER(\%)↓} & \textbf{$\Delta$ WER(\%)↓} & \textbf{CER(\%)↓} & \textbf{$\Delta$ CER(\%)↓} \\
    \midrule
    \multirow{8}{*}{mWhisper-Flamingo \cite{mWhisper-Flamingo}} 
      & \multirow{8}{*}{LRS3 \cite{lrs3}} 
      & \multirow{4}{*}{A} & \multirow{4}{*}{En} 
      & Offline & 0.68 & * & * & * \\
      &  &  &  & Zoom  & 10.38 & 9.70 & * & * \\
      &  &  &  & Lark  & 19.55 & 18.87 & * & * \\
      &  &  &  & Tencent Meeting  & 11.89 & 11.21 & * & * \\
      \cmidrule(lr){3-9}
      &  & \multirow{4}{*}{AV} & \multirow{4}{*}{En}  & Offline & 0.73 & * & * & * \\
      &  &  &  & Zoom  & 9.22 & 8.49 & * & * \\
      &  &  &  & Lark  & 18.53 & 17.80 & * & * \\
      &  &  &  & Tencent Meeting  & 10.97 & 10.24 & * & * \\
    \midrule
    \multirow{8}{*}{LiPS-AVSR \cite{LiPS-AVSR}} 
      & \multirow{8}{*}{Chinese-Lips \cite{LiPS-AVSR}} 
      & \multirow{4}{*}{A} & \multirow{4}{*}{Zh} 
      & Offline & * & * & 4.37 & * \\
      &  &  &  & Zoom  & * & * & 8.67 & \textbf{4.30} \\
      &  &  &  & Lark  & * & * & 14.83 & 10.46 \\
      &  &  &  & Tencent Meeting  & * & * & 9.72 & 5.35 \\
      \cmidrule(lr){3-9}
      &  & \multirow{4}{*}{AV} & \multirow{4}{*}{Zh} & Offline & * & * & 3.87 & * \\
      &  &  &  & Zoom  & * & * & 18.53 & 14.66 \\
      &  &  &  & Lark  & * & * & 10.97 & 7.10 \\
      &  &  &  & Tencent Meeting  & * & * & 9.22 & 5.35 \\
    \midrule
    \multirow{12}{*}{Auto-AVSR \cite{auto-avsr-2}} 
      & \multirow{8}{*}{LRS3 \cite{lrs3}} 
      & \multirow{4}{*}{AV} & \multirow{4}{*}{En} 
      & Offline & 0.93 & * & 0.56 & * \\
      &  &  &  & Zoom  & 33.09 & 32.16 & 33.01 & 32.45 \\
      &  &  &  & Lark  & 31.72 & 30.79 & 30.71 & 30.15 \\
      &  &  &  & Tencent Meeting  & 23.79 & 22.86 & 22.65 & 22.09 \\
      \cmidrule(lr){3-9}
      & 
      & \multirow{4}{*}{V} & \multirow{4}{*}{En} 
      & Offline & 19.08 & * & 13.68 & * \\
      &  &  &  & Zoom  & 90.26 & 71.18 & 74.32 & 60.64 \\
      &  &  &  & Lark  & 92.08 & 73.00 & 74.51 & 60.83 \\
      &  &  &  & Tencent Meeting  & 56.14 & 37.06 & 43.88 & 30.20 \\
      \cmidrule(lr){2-9}
      & \multirow{4}{*}{Lombard-Grid \cite{lombard_grid}} 
      & \multirow{4}{*}{AV} & \multirow{4}{*}{En} 
      & Offline & 4.93 & * & 3.06 & * \\
      &  &  &  & Zoom  & 12.36 & \textbf{7.43} & 9.93 & 6.87 \\
      &  &  &  & Lark  & 8.94 & \textbf{4.01} & 7.79 & \textbf{4.73} \\
      &  &  &  & Tencent Meeting  & 7.12 & \textbf{2.19} & 4.48 & \textbf{1.42} \\
    \bottomrule
  \end{tabular}
  }
\end{table*}

With the spread of the COVID-19 pandemic, VC has become commonplace, whereas it was previously a relatively niche practice. AVSR models are often deployed on VC platforms to transcribe the meeting content. Existing AVSR models are typically trained on clean datasets, and artificial noise is later added during post-processing to improve model robustness. However, real-world VC scenarios involve multiple complex factors, including codec compression, transmission delays, and speech enhancement effects. This section aims to systematically evaluate the performance of existing SOTA models under VC conditions.

\subsection{Setup}\label{setup}
To comprehensively evaluate the performance of current AVSR models under VC conditions, we employed three representative VC platforms and evaluated three SOTA AVSR models across multiple datasets and languages. 

\subsubsection{Dataset}
Considering the linguistic differences, we selected both English and Chinese multimodal datasets, specifically Lombard-Grid \cite{lombard_grid}, LRS3 \cite{lrs3}, and Chinese-Lips \cite{LiPS-AVSR}. 

% Lombard-Grid is a multimodal corpus covering both frontal and profile views, consisting of 5400 video samples from 54 speakers, including 2700 Lombard and 2700 plain reference utterances, with each video following the standardized sentence structure of the original “Grid” corpus. The LRS3 dataset contains over 400 hours of face tracks extracted from TED and TEDx talks, along with their corresponding textual transcriptions. Chinese-Lips is a Chinese multimodal audio-visual dataset comprising 100 hours of facial video clips paired with their corresponding sentence transcriptions.

\subsubsection{Baselines}
To evaluate the performance of AVSR models in VC, we selected three SOTA models, specifically Auto-AVSR \cite{auto-avsr-2}, mWhisper-Flamingo \cite{mWhisper-Flamingo}, and LiPS-AVSR \cite{LiPS-AVSR}. 
% Auto-AVSR is trained on the Lombard-Grid and LRS3 datasets. mWhisper-Flamingo is built upon the LRS3 dataset. LiPS-AVSR is trained on the Chinese-Lips dataset. 

\subsection{Metrics}
We adopt Word Error Rate (WER) and Character Error Rate (CER) as metrics. Lower WER and CER values indicate better performance.

\subsubsection{Video Conferencing Platform}
With the widespread adoption of VC, various applications have rapidly emerged. We selected several commonly used platforms, including Zoom, Lark, and Tencent Meeting. 

\subsection{Evaluation Method}
To ensure a fair comparison of baselines across different platforms, we followed the open-source configurations of each baseline, successfully reproducing their performance with results closely matching those reported in the original papers. Furthermore, we transmitted the test sets of each corresponding dataset through the VC platforms to simulate the VC conditions. We provide a detailed description of the transmission process in Appendix 8.1. We then computed the WER and CER on the transmitted test sets to evaluate the performance of each baseline. 

\subsection{Quantitative Results} \label{previous_results}
\subsubsection{Performance Analysis}
% We present the quantitative results in Tab. \ref{avsr-results} and visualize the WER/CER increment caused by video conferencing transmission as heatmaps in Fig. \ref{increase}. 

We present the quantitative results in Tab. \ref{avsr_results}. The results reveal that all models suffer significant performance degradation under VC conditions. This degradation remains consistent across different languages and modalities, confirming the destructive impact of VC on AVSR models. mWhisper-Flamingo exhibits a significant performance decline when deployed in VC compared to its offline baseline. On the LRS3 dataset, the WER of mWhisper-Flamingo in audio-only modality increases by an average of 20.5 times compared to the offline setting. Although the audio-visual modality variant slightly mitigates the degradation (WER = 9.22\% on Zoom vs. 10.38\% in audio-only), the overall accuracy remains significantly lower than that of the offline condition. 

For LiPS-AVSR, the degradation pattern is consistent. The offline CER of 4.37\% (audio-only) and 3.87\% (audio-visual) nearly doubles or triples under conferencing conditions. Notably, the audio-visual configuration suffers substantial instability, reaching up to 18.53\% on Zoom. This suggests that visual cues may be unreliable when video compression or transmission delay occurs.

The Auto-AVSR model exhibits the most pronounced performance degradation among the three evaluated systems. On the LRS3 dataset, the WER of Auto-AVSR in audio-visual modality increases from 0.93\% to 33.09\%. In contrast, the audio-visual evaluation on the Lombard-Grid dataset shows relatively minor degradation, indicating that Auto-AVSR trained with Lombard data is more resilient to VC distortions. Through the comparison between the Lombard-Grid and LRS3 datasets, it can be observed that the model trained on Lombard data is inherently more stable under conferencing conditions.

\subsubsection{Modal Analysis}
Different modality combinations exhibit markedly distinct levels of tolerance to VC conditions, which directly determine the robustness of AVSR models. Among them, the visual-only modality is the most vulnerable, as all datasets show severe performance degradation under VC scenarios. For instance, in the Lark of the LRS3 dataset, the Auto-AVSR model achieves a WER of 92.08\%, while in the Zoom it reaches 90.26\%. These results indicate that the visual-only modality is more sensitive to compression and delay during transmission, making it difficult for a vision-only system to resist such distortions. 

Audio-only modality exhibits moderate robustness, with the WER/CER increases of the mWhisper-Flamingo and LiPS-AVSR models under VC conditions being lower than those of the audio-visual modality. For instance, in the LRS3 dataset under Zoom transmission, the mWhisper-Flamingo model achieves a WER of 10.38\% in audio-only modality, higher than 9.22\% in audio-visual modality. 

Audio-visual modality exhibits the strongest robustness. In most cases, the audio-visual modality of baseline models effectively mitigates interference in VC scenarios through cross-modal information complementarity. For the Auto-AVSR model on the LRS3 dataset, the AV fusion modality achieves a maximum WER of 33.09\% in VC scenarios, which is substantially lower than the 92.08\% observed in the visual-only modality. The audio-visual modality of the mWhisper-Flamingo model achieves lower WER than the audio-only modality across all three platforms.

\subsubsection{Dataset Analysis}
The inherent characteristics of different datasets (such as video quality, speaker diversity, and data distribution) directly affect the extent of performance degradation after transmission. Among them, the Lombard-Grid dataset shows the most substantial resistance to interference. For the Auto-AVSR model on this dataset, the WER under the audio-visual modality remains as low as 12.36\% even after transmission via Zoom, which is substantially lower than the 33.09\% WER observed for the same modality on the LRS3 dataset. In addition, the model trained on Lombard-Grid exhibits the smallest increases in WER and CER across nearly all settings. The primary reason lies in the fact that half of the data in Lombard-Grid exhibits the Lombard effect. Previous studies \cite{lombard_avsr_1, lombard_avsr_2} have confirmed that training AVSR models on data containing the Lombard effect can simultaneously improve recognition accuracy and robustness.

\subsection{Summary of Findings}\label{findings}
We evaluated several AVSR models across mainstream VC platforms. We found that the performance degradation of AVSR models is a pervasive issue, regardless of model architecture, language, modality, or VC platform. Interestingly, we observed that models trained with Lombard data exhibit strong robustness in VC.








==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/4_dataset.tex <==
\section{Multimodal Dataset for Video Conferencing}
The previous section revealed that AVSR models degrade notably in VC. However, existing datasets fail to capture the unique characteristics of such scenarios. In this section, we identify two key factors of VC scenarios and construct the first multimodal VC dataset for AVSR (MLD-VC), which explicitly incorporates these two key factors.
\subsection{Key Factors of Video Conferencing}
According to the previous analysis, we identify two key factors of VC scenarios, as shown in Fig.~\ref{application}. \textbf{(K1) Transmission distortions.} Compared to offline scenarios, audio-visual signals in VC are subject to complex interferences, including codec compression, noise suppression, and speech enhancement processing. These external interferences degrade the clarity and intelligibility of both audio and visual streams. \textbf{(K2) Spontaneous human hyper-expression.} Beyond distortion, human behavior in VC differs from offline scenarios. Psychoacoustic and auditory studies \cite{hyper_1,hyper_theory,lombard_3} have demonstrated that speakers, under conditions of communicative obstruction, spontaneously enhance their vocal expressions and facial articulations to ensure effective information transmission. This phenomenon, termed “Hyper-expression”, manifests as a slower speech rate, expanded vowel articulation space, and more pronounced lip and head movements. Previous studies \cite{hyper_1} have confirmed the widespread presence of such hyper-expression behaviors in VC. Since the Lombard effect is a typical form of hyper-expression \cite{hyper_theory}, this finding explains why the models trained with Lombard data in Section \ref{findings} exhibit stronger robustness in VC.

Under the combined influence of \textbf{K1} and \textbf{K2}, the data distribution in VC deviates significantly from that of “clean” in offline conditions. For AVSR models trained on offline data, these two key factors directly cause a severe degradation in model performance.

\subsection{Dataset Construction}
\subsubsection{Participant information and consent}
We recruited a total of 31 volunteers to participate in the data collection process, all of whom were university students, including 15 males and 16 females. Each participant was fully informed about the research objectives, data recording procedures, and the specific types of personal information retained (e.g., age and gender). All participants were required to sign an informed consent form that clearly stated the intended use of the collected data. After the data collection, participants were asked to review all recorded audio-visual materials for verification. The final released dataset will undergo a rigorous anonymization process to ensure participant privacy.
\subsubsection{Core of Dataset}\label{innovation}
To better highlight the characteristics of VC, we systematically incorporate \textbf{K1} and \textbf{K2} in the proposed dataset. To faithfully reproduce transmission distortions under VC conditions, we select several widely used platforms, including Tencent Meeting, Lark, DingTalk, and Zoom. Previous studies \cite{hyper_1} have shown that hyper-expression behaviors in VC are highly analogous to the Lombard effect. The Lombard effect \cite{lombard_avsr_1, lombard_avsr_2} is induced by environmental noise, and its intensity varies in relation to the level of noise exposure. Therefore, we introduce controlled noise stimuli to elicit the Lombard effect in speakers, thereby enhancing the representativeness of hyper-expression phenomena in VC.

By incorporating the two key factors of VC, our constructed dataset more accurately aligns with the signal properties and human interaction patterns of VC. This dataset can make a new contribution to investigating the degradation mechanisms and enhancing the robustness of AVSR models under VC conditions.

\subsubsection{Corpus Design}
We designed both an English and a Chinese corpus. The sentence construction was inspired by the Lombard-Grid dataset (English) \cite{lombard_grid} and the DB-MMLC dataset (Chinese) \cite{lombard_2}, both of which adopt the Grid-style grammar. Each English sentence in our dataset consists of six words. For example, “bin blue at A 2 please” follows the structure:
\textless Command: bin, lay, place, set\textgreater \textless Color: blue, green, red, white\textgreater \textless Preposition: at, by, in, with\textgreater  \textless Letter: A–Z (excluding W)\textgreater \textless Digit: 0–9\textgreater \textless Adverb: again, now, please, soon\textgreater. Among them, three words (color, letter, and digit) are regarded as keywords, while the remaining ones are considered fillers. The Chinese version of the Grid-style corpus used in our dataset is provided in Appendix 8.2.1.

To introduce the Lombard effect, we followed previous studies and designed four background noise conditions, including Plain (no noise), 40 dB, 60 dB, and 80 dB. All participants were informed that they were taking part in a video conference. They were required to wear headphones, sit in front of a display and camera, and read aloud the sentences from the corpus. The display prompted participants to start reading, while the corresponding background noise was simultaneously played through the headphones. Participants were required to complete the reading task under each of the noise conditions. Each participant was required to read 30 sentences (20 Chinese sentences and 10 English sentences) under each of the four background noise conditions. 

\subsubsection{Recording} \label{recording}
To simulate real-world usage scenarios, all VC platforms were configured with their default settings. The audio and video input devices consisted of a UGREEN CM564 microphone and a UGREEN CM831-65381 camera. Both the input and receiving audio–video streams were recorded using OBS Studio. The recording parameters of OBS Studio were set as follows: stereo audio with a 48 kHz sampling rate encoded using the AAC codec, and video with a resolution of 1920 × 1080 at 25 FPS. The recordings from the input side were treated as offline data, while those from the receiving side were regarded as VC data.

\subsubsection{Post Processing}
To improve the quality of the dataset, we manually inspected the recorded raw data and discarded any “corrupted samples” caused by unexpected recording issues. To ensure anonymization, we followed the preprocessing configuration of Auto-AVSR \cite{auto-avsr-2} and cropped each video to retain only the lip region. To eliminate the influence of system volume during recording, we applied loudness normalization to the audio. To ensure compatibility with various AVSR model inputs, we used FFMPEG to convert all audio into single-channel WAV files with a sampling rate of 16 kHz.

\subsection{Dataset Distribution}
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[t]
  \centering
    \caption{
    Comparison of the proposed MLD-VC with existing multimodal Lombard and video conferencing datasets. “VC Num” refers to the number of video conferencing platforms included. “*” indicates that the dataset was collected offline.
  }
  \resizebox{\linewidth}{!}{
    \begin{tabular}{cccccc}
    \toprule
    \textbf{Dataset} & \textbf{Speakers} & \textbf{Duration(h)} & \textbf{Language} & \textbf{VC Num} & \textbf{Year} \\
    \midrule
    Lombard-Grid & 54    & 3.81     & En    & * & 2018 \\
    RoomReader & \textbf{118 }  & 8     & En    & 1  & 2022 \\
    \textbf{MLD-VC (Ours)}  & 31    &\textbf{ 22.79}    & \textbf{En \& Zh} & \textbf{4} & \textbf{2025} \\
    \bottomrule
    \end{tabular}%
  \label{dataset_compare}%
  }
\end{table}%

Tab. \ref{dataset_compare} compares our dataset with existing multimodal Lombard datasets and video conferencing datasets. Our dataset substantially extends the total duration and the number of platforms compared with existing datasets. Compared to RoomReader, our dataset is 2.8 times longer in total duration and encompasses three additional VC platforms. Compared with Lombard-Grid, our dataset is more than 6 times longer in total duration and extends to the online scenario. Additionally, our dataset supports multiple languages and various VC platforms. We present the duration of each subset across different VC platforms in Appendix 8.2.3.



==> sec/5_analysis.tex <==
\section{Revealing the Cause of AVSR Degradation}
In the previous results presented in Section \ref{previous_results}, we observed a significant performance degradation of AVSR models in VC. This phenomenon suggests that both the audio-visual features undergo distributional shifts under VC conditions, resulting in impaired performance. To further investigate this issue, we conducted a systematic analysis of audio-visual data in the proposed MLD-VC dataset. We compared the characteristics of audio and visual modalities between offline and online settings, revealing the direct manifestations of AVSR performance degradation. In addition, we dissected the transmission and processing pipeline in VC systems to identify the critical stages responsible for modality distribution shifts, thereby uncovering the underlying causes of AVSR performance deterioration. 

\subsection{Analysis of Modality Difference}
To analyze the modality discrepancies across different scenarios, we visualize the probability density distributions of representative features. For the audio modality, we use openSMILE \cite{eyben2010opensmile} to extract five acoustic features: the fundamental frequency (F0), the first formant (F1), the second formant (F2), loudness, and the ratio of the total energy in the 50-1kHz to the total energy in the 1kHz-5kHz (AlphaRatio). Note that the values of AlphaRatio are logarithmically scaled. 

For the visual modality, compression and network latency in online transmission inevitably cause quality degradation and even blurring. Traditional image quality measures, such as PSNR and SSIM, have limited value in this scenario because they cannot capture the information that AVSR models primarily rely on. The essential objective of AVSR is to recognize lip movements. Based on this task property, we use lip geometric motion as the primary target for analysis. Specifically, we use three indicators: lip width, lip height, and lip roundness. Lip roundness is defined as the ratio between height and width, and a value closer to 1 indicates a more rounded lip shape. All indicators are computed from facial landmark positions, and the detailed procedure is provided in Appendix 8.3.1.

\subsubsection{Difference between Offline and Online}
We present the probability density curves of speech features in Fig. \ref{audio_analysis}. In addition, Tab. \ref{peak_x_coordinates} lists the horizontal coordinates corresponding to the peak points of each curve. We find that the F0 remains nearly consistent across offline and online scenarios, indicating that the overall pitch level of speech is not substantially affected. In contrast, both F1 and F2 exhibit significant upward frequency shifts, with DingTalk showing the approximate 170 Hz increase. AlphaRatio in online settings is lower than in offline settings, indicating that high-frequency energy is enhanced in online recordings. Moreover, the loudness distribution shifts to the left in online scenarios, suggesting a slight attenuation in overall acoustic energy. These patterns are consistent across all VC platforms, indicating that VC platforms systematically alter the spectral structure of audio, thereby impairing the accurate modeling of features by AVSR models.

\subsubsection{Difference between Plain and Hyper-expression}
We use the Lombard effect to enhance the hyper-expression in VC explicitly. By comparing the paired subplots (row-wise) in Fig. \ref{audio_analysis} with the corresponding sub-tables in Tab. \ref{peak_x_coordinates}, it can be observed that the F0 remains essentially unchanged under the Lombard condition. At the same time, the distributions of the F1 and F2 shift toward higher frequencies with reduced dispersion. We further observe that the variations of F1 and F2 between Plain and Lombard speech resemble those between offline and online recordings, indicating that the spectral structures induced by the Lombard effect are similar to those of video conferencing. This finding explains why the model trained with Lombard data in Section \ref{findings} shows stronger robustness in VC.

\subsubsection{Difference between Audio and Vision}
We present the visual feature analysis results in Appendix 8.3.2. The results show that the differences in visual features are minimal, indicating that the VC scenario exerts only a negligible influence on lip landmarks. However, this does not imply that the degradation in AVSR performance is unrelated to the visual modality. We observe that Auto-AVSR, mWhisper-Flamingo, and LiPS-AVSR employ pre-trained ResNet18 \cite{resnet18} and AVHuBERT \cite{shi2022avhubert} backbones to process visual inputs. Moreover, these models take lip images rather than lip landmarks as visual inputs. Due to codec compression, transmission delay, and other factors, lip images are subject to distortion, resulting in a distributional shift in the visual modality. In contrast, our analysis indicates that landmark-level features remain stable in VC, suggesting that future AVSR models could benefit from geometry-based visual encodings.
\begin{figure}[t]
  \centering
   \includegraphics[width=1\linewidth]{sec/pictures/audio_modal_analysis.pdf}
\caption{
Probability density curves of five acoustic features (F0, F1, F2, Loudness, and AlphaRatio) across five subsets in the proposed MLD-VC under \textit{Plain} (left column) and \textit{Lombard} (right column).
Across features(column-wise), both \textit{Plain} and \textit{Lombard} show noticeable high-frequency shifts in F1 and F2 under video conferencing conditions.
Across conditions (row-wise), \textit{Lombard} also exhibits overall higher F1 and F2 than \textit{Plain}.
}
   \label{audio_analysis}
\end{figure}


\begin{figure}[t]
  \centering
   \includegraphics[width=1\linewidth]{sec/pictures/problem_location.pdf}
   \caption{
Illustration of how video conferencing platforms affect speech formants.
We simulate platform processing by applying OPUS compression and three typical speech enhancement algorithms.
The four subplots show F1 and F2 distributions before and after processing.
Only the enhancement stages introduce noticeable spectral shifts and formant distortions, which explain the frequency bias observed in real video conferencing recordings.
}
\label{problem_location}
\end{figure}


\subsection{Identifying the Source of Distribution Drift}
\begin{table}[t]
\centering
\caption{Peak abscissas of probability density curves for different acoustic features.}
\label{peak_x_coordinates}
\resizebox{\linewidth}{!}{%
\begin{tabular}{cccccc}
\toprule
\multirow{2}{*}{\textbf{Acoustic Feature}} & \multicolumn{5}{c}{\textbf{Platform}} \\
\cmidrule(lr){2-6}
 & \textbf{Offline} & \textbf{Tencent Meeting} & \textbf{Lark} & \textbf{DingTalk} & \textbf{Zoom} \\
\midrule
F0 (\textit{Plain}) & 37.28  & 37.66  & 37.51  & 37.66  & 37.39  \\
F0 (\textit{Lombard})  & 37.58  & 37.85  & 37.62  & 37.64  & 37.55  \\
\midrule
F1 (\textit{Plain}) & 606.90  & 674.43  & 704.19  & 774.61  & 687.88  \\
F1 (\textit{Lombard})  & 660.06  & 756.11  & 770.17  & 825.44  & 712.73  \\
\midrule
F2 (\textit{Plain}) & 1655.66  & 1680.78  & 1727.37  & 1783.51  & 1727.45  \\
F2 (\textit{Lombard})  & 1665.07  & 1832.85  & 1863.88  & 1829.73  & 1746.69  \\
\midrule
Loudness (\textit{Plain}) & 0.88 & 0.68 & 0.69 & 0.68 & 0.68 \\
Loudness (\textit{Lombard})  & 0.86 & 0.72 & 0.73 & 0.67 & 0.68 \\
\midrule
AlphaRatio (\textit{Plain}) & -12.12 & -13.19 & -13.67 & -12.52 & -14.59 \\
AlphaRatio (\textit{Lombard})  & -8.81 & -10.07 & -8.67 & -8.28 & -10.47 \\
\bottomrule
\end{tabular}%
}
\end{table}

After analyzing Fig. \ref{audio_analysis}, we found that several acoustic features exhibited noticeable shifts under VC conditions. In particular, under the Plain condition, although hyper-expression occurred in the VC scenario, the shifts in F1 and F2 were significantly larger than those caused by hyper-expression. Therefore, we believe that the hyper-expression does not solely cause the pronounced deviations in F1 and F2 but is also likely influenced by the audio processing applied in the VC platforms.

To identify the underlying causes, we systematically deconstructed the speech processing pipeline in the VC scenario. Typically, the original speech undergoes codec compression and speech enhancement before being transmitted to the receiver. Since VC platforms operate as a black box, we can only approximate the process to locate the stages responsible for the acoustic feature shifts. We used the OPUS codec, which is widely adopted in VC platforms, such as Zoom, to simulate the codec compression stage. In addition, we employed Sepformer \cite{sepformer}, NoiseReduce \cite{noisereduce}, and DeepFilterNet \cite{schroeter2023deepfilternet3} as speech enhancement methods to model the enhancement stage in VC. The offline samples in MLD-VC were processed through codec compression and speech enhancement individually, and the resulting changes in their F1 and F2 were analyzed and compared.

Following the settings in Fig. \ref{audio_analysis}, we present the results in Fig. \ref{problem_location}. We observe that the codec compression stage has minimal impact on F1 and F2, with their frequency distributions remaining stable. In contrast, speech enhancement leads to an overall upward shift of F1 and F2. This phenomenon closely resembles the patterns observed in the real VC scenario illustrated in Fig. \ref{audio_analysis}. Therefore, we conclude that speech enhancement primarily causes the acoustic abnormalities in VC speech. While these algorithms improve the intelligibility, they also alter the spectral structure of speech. Consequently, these changes degrade the performance of AVSR. This finding reveals an essential cause of performance degradation in AVSR within the VC scenario from an acoustic perspective.

==> sec/6_finetune.tex <==
\section{Performance Evaluation on MLD-VC}
\subsection{Experiment Setup}
To further investigate the impact of MLD-VC for VC, we fine-tuned the AVSR model using the proposed MLD-VC dataset and evaluated its performance across different VC platforms. We followed the experimental setup described in Section \ref{setup} and utilized the LiPS-AVSR model \cite{LiPS-AVSR} for fine-tuning. The MLD-VC dataset was divided into training and testing sets. Additionally, ablation experiments were conducted to assess the contribution of online data and hyper-expression data to model performance. We present the implementation details in Appendix 8.4.
% \subsection{Implement Detials}

\subsection{Fine-tuning Results}
\begin{table}[t]
  \centering
  \caption{Results of fine-tuning with MLD-VC dataset on AVSR performance under video conferencing conditions. “*” indicates that the corresponding metric is not applicable or not reported.}
  \resizebox{\linewidth}{!}{
  \begin{tabular}{lcccc}
    \toprule
    \textbf{Test Dataset} & \textbf{Platform} & \textbf{Finetune} & \textbf{CER(\%)↓} & \textbf{Reduction(\%)} \\
    \midrule
    \multirow{6}{*}{Chinese-Lips \cite{LiPS-AVSR}} 
      & Tencent Meeting   & × & 10.97 & * \\
      & Tencent Meeting   & \checkmark & \textbf{9.65} & \textbf{12.0} \\
      & Lark & × & 18.53 & * \\
      & Lark & \checkmark & \textbf{13.64} & \textbf{26.4} \\
      & Zoom & × & 9.22 & * \\
      & Zoom & \checkmark & \textbf{7.93} & \textbf{14.0} \\
    \midrule
    \multirow{2}{*}{MLD-VC (Ours)} 
      & * & × & 42.37 & * \\
      & * & \checkmark & \textbf{13.91} & \textbf{67.2} \\
    \bottomrule
  \end{tabular}
  \label{tab:finetune}
  }
\end{table}

Tab.~\ref{tab:finetune} presents the fine-tuning results. We observed that models fine-tuned with MLD-VC achieved improved recognition accuracy across all VC platforms. Specifically, the fine-tuned models achieved an average relative reduction of 17.5\% in the CER across the three platforms. Furthermore, the CER on the MLD-VC test set decreased by 67.2\% after fine-tuning. This substantial improvement indicates that the fine-tuned models not only improve in-domain performance but also significantly enhance cross-platform generalization. These results highlight the effectiveness of MLD-VC for AVSR models in VC.

\subsection{Ablation}
\begin{table}[t] 
\footnotesize
  \centering
  \caption{Ablation study on the effects of online data and hyper-expression in MLD-VC fine-tuning. The results show that both online recording conditions and hyper-expression samples significantly contribute to lowering the CER.}
  \resizebox{\linewidth}{!}{
  \begin{tabular}{ccccc}
    \toprule
    \textbf{Online} & \textbf{Hyper-expression} & \textbf{Tencent Meeting} & \textbf{Lark} & \textbf{Zoom} \\
    \midrule
    \checkmark & \checkmark & \textbf{9.65} & \textbf{13.64} & \textbf{7.93} \\
    × & \checkmark & 10.15 & 15.52 & 10.53 \\
    \checkmark & × & 10.01 & 14.48 & 9.61 \\
    \bottomrule
  \end{tabular}
  \label{tab:ablation}
}
\end{table}

To better understand the contribution of different data components within the proposed MLD-VC dataset, we conduct an ablation study focusing on two key factors: (1) transmission distortions (online vs. offline) and (2) spontaneous human hyper-expression. 

The ablation results are summarized in Tab.~\ref{tab:ablation}. When online data were excluded, the average CER across VC platforms increased by 15.9\%. When hyper-expression data were excluded, the average CER increased by 10.5\%. These results indicate that both realistic recording conditions and spontaneous hyper-expressions are indispensable for improving the robustness of AVSR in VC scenarios. The combination of the two enables models to generalize more effectively to real-world VC conditions, validating the design rationale of the MLD-VC dataset discussed in Section \ref{innovation}.

==> sec/7_conclusion.tex <==
\section{Conclusion}
We present the first systematic investigation of AVSR in real-world video conferencing. Our study reveals that transmission distortions and spontaneous human hyper-expression jointly lead to drastic performance degradation. Through detailed analysis, we identify speech enhancement algorithms as the primary source of distribution shift, which alters the F1/F2 formants. Moreover, we find that the distributional characteristics induced by the Lombard effect closely resemble those caused by speech enhancement, which explains why Lombard-trained models exhibit superior robustness in video conferencing. To bridge the gaps of lack of video conferencing data, we construct \textbf{MLD-VC}, the first multimodal dataset tailored for video conferencing, explicitly modeling hyper-expression under realistic online recording conditions. Fine-tuning AVSR models on MLD-VC achieves a 17.5\% average reduction in CER across platforms, and ablation studies confirm that both transmission distortions and hyper-expression data are crucial for improving the robustness of AVSR in video conferencing.

\section{Acknowledgement}
This work is supported in part by the National Natural Science Foundation of China (NO.62572358, NO.62172306, NO.62372334) and  DiDi Chuxing Group.
